Koopman-LQR Controller for Quadrotor UAVs from Data

Quadrotor systems are common and beneficial for many fields, but their intricate behavior often makes it challenging to design effective and optimal control strategies. Some traditional approaches to nonlinear control often rely on local linearizations or complex nonlinear models, which can be inaccurate or computationally expensive. We present a data-driven approach to identify the dynamics of a given quadrotor system using Koopman operator theory. Koopman theory offers a framework for representing nonlinear dynamics as linear operators acting on observable functions of the state space. This allows to approximate nonlinear systems with globally linear models in a higher dimensional space, which can be analyzed and controlled using standard linear optimal control techniques. We leverage the method of extended dynamic mode decomposition (EDMD) to identify Koopman operator from data with total least squares. We demonstrate that the identified model can be stabilized and controllable by designing a controller using linear quadratic regulator (LQR).

==> sections/methodology_old.tex <==
\subsection{Koopman operator theory}

\begin{definition} [Koopman Operator] Consider the discrete time dynamical system
\begin{equation} \label{eq:dynamics}
    x^{+}_{k} = {f}({x_{k}, u_{k}}),
\end{equation}
where ${x}_{k} \in \mathbb{R}^n$  is a state vector of the system, ${u}_{k} \in \mathbb{R}^{l}$ is the control input vector at time $k$, ${f}$ is a transition map such that $f: \mathbb{R}^n \times \mathbb{R}^l \mapsto \mathbb{R}^n$, and $x^{+}$ is the successor state of the system. The Koopman operator $\mathcal{K}_t$ is an infinite dimensional operator \begin{equation*}\label{eq:koop_def}
\mathcal{K}_t \xi = \xi \circ f(x_k, u_k).
\end{equation*}
acts on $\xi \in \mathcal{H}: \mathbb{R}^n \times \mathbb{R}^l \mapsto \mathbb{R}$, the observable functions of the state space, where $\circ$ is the function composition operator. \hfill $\Box$
\end{definition} 
The Koopman operator acts on the Hilbert space $\mathcal{H}$ of all scalar measurement functions $\xi$ and is by definition a \textit{linear operator}--since for $\xi_1, \xi_2 \in \mathcal{H}$ and $\alpha_1, \alpha_2 \in \mathbb{R}$
\begin{equation}
    \begin{aligned}
    \mathcal{K}_t(\alpha_1 \xi_1, \alpha_2 \xi_2) &= \alpha_1 \xi_1 \circ f + \alpha_2 \xi_2 \circ f\\
    &= \alpha_1 \mathcal{K}_t \xi_1 + \alpha_2 \mathcal{K}_t \xi_2,
\end{aligned}
\end{equation}

It, thus, provides a linear formulation of a nonlinear system, but in the infinite dimensional space $\mathcal{H}$ of the observable functions \cite{budivsic2012applied}. Therefore, nonlinear, finite-dimensional dynamics are traded for linear, infinite-dimensional dynamics in the transformation from the state-space representation of the dynamical system to the Koopman representation. However, from practical point of view we are interested in a finite representation of the Koopman operator.  In our settings, this will be done using the concept of DMD.

One attractive advantage of the linear systems from control theory perspective is to have a convex search space for the cost function of the well known controllers such as LQR and MPC (see figure \ref{fig:koopman_illustration}).


\begin{figure}[]
    \centering
    \includegraphics[width = 0.5\textwidth]{figures/figures_Koopman.pdf}
    \caption{Pictorial illustration of the Koopman Operator: Koopman Operator ($\mathcal{K}_t$) maps the state-space into lifted linear space and acts on the function space governed by ${\xi}$. The {\color{green}{green}} panels represent linear space which corresponds to convex search space when it comes to control design. On the other hand, the {\color{red}{red}} panels is the generic nonlinear state-space which corresponds to non-convex search space for control design which leads to sub-optimal control.}
    \label{fig:koopman_illustration}
\end{figure}
% Dynamic mode decomposition is a matrix decomposition technique that might offer a data-driven finite-dimension approximation of the Koopman operator $\mathcal{K}$ which linearize the system globally \cite{schmid2010dynamic, tu2013dynamic}. In that sense, the choice of the observables is a critical and will affect the discovered operator \cite{williams2015data}.
\subsection{Approximation of Koopman Operator using Dynamic Mode Decomposition with Control}
We look forward to approximating the Koopman operator from data as a way to overcome the challenges of its infinite dimensionality. Consider a carried out experiment for the system in (\ref{eq:dynamics}) and its states and input data are recorded in the following way
\begin{align*}
    \mathcal{D} := \{x_k, u_k: k \in [0, (T-1)T_s]\cap\mathbb{Z}_{0}\},
\end{align*}
\begin{assumption} \label{ass:D}
    The set $\mathcal{D}$ exists. \hfill $\Box$
\end{assumption}
Let assumption \ref{ass:D} holds. Then, we define
\begin{subequations}
\begin{align}
    &\Gamma:= \mat{u(0)~ u(T_s)~ \dots ~ u((T-1)T_s)} \in \mathbb{R}^{l \times T},\\
    &X:= \mat{x(0)~ x(T_s)~ \dots~ x((T-1)T_s)} \in \mathbb{R}^{n \times T},\\
    & X^{+} := \mat{x(1)~ x(T_s)~ \dots~ x((T)T_s)} \in \mathbb{R}^{n \times T}.
\end{align}
\end{subequations}
\begin{assumption} \label{ass:PE}
    Considering $T \geq n+l $, the matrix $\mat{X\\ \Gamma}$ has full row rank.\hfill  $\Box$
\end{assumption}
\begin{definition}[DMD] \label{def:DMD}
    Consider a dynamical system ${x}^{+}_{k} = {f}({x}_k, {u}_k) \approx {A}{x}_k + {B} {u}_k $ and dataset $\mathcal{D}$. The system can be written as
    \begin{align} 
        {X}^{+} &= {A}{X} + {B}{\Gamma}\\
        &= \begin{bmatrix}
            {A} ~ {B}
        \end{bmatrix} \begin{bmatrix}
            {X}\\ {\Gamma}
        \end{bmatrix} = \hat{\mathcal{K}_t} {\Omega}
        \label{eq:dmdc}
    \end{align}
    Let assumption \ref{ass:PE} hold, the solution to (\ref{eq:dmdc}) can be solved using
    \begin{align}
    \label{eq:soln_ls}
        {\hat{\mathcal{K}_t}} = \argmin_{{\hat{\mathcal{K}_t}}} ||{X^{+}} - {\hat{\mathcal{K}_t}} \Omega||_{\text{F}} = {X^{+}}{\Omega}^{\dagger},
    \end{align}
    where $({\cdot})^{\dagger}$ denotes the Moore-Penrose pseudo-inverse, $\|\cdot\|_{\text{F}}$ denotes the Frobenius norm, and $\hat{\mathcal{K}_t}$  is an approximation for the Koopman operator. \hfill  $\Box$
\end{definition}
\begin{remark}
    The Moore-Penrose pseduo-inverse is calculated using singular value decomposition (SVD).\hfill  $\Box$
\end{remark}
The original DMD algorithm was developed for non-controlled system \cite{schmid2010dynamic} then in \cite{proctor2016dynamic}, the authors extended the algorithm to account for controlled settings. For readers who are interested in DMD we refer to \cite{schmid2010dynamic, tu2013dynamic} for more elaborate discussion.

From definition \ref{def:DMD}, DMD can be extended by lifting the states into higher dimensional space using EDMD by defining the observable functions discussed earlier. The main deference between the nominal DMD and EDMD is that the observables in the nominal case are simple identity map. The EDMD algorithm can be used to somehow, if the observable function are chosen wisely (i.e. chosen to be invariant under the Koopman operator), to account for complex nonlinearities by having an exact Koopman operator identification. Otherwise, the used observable functions can result in approximated Koopman operator. If the observable functions are not Koopman invariant (e.g. Koopman eigen-functions), they can be found either by brute-force trial and error in a specific basis for Hilbert space (e.g., trying numerous polynomial functions, or Fourier basis functions) or by prior knowledge about the system. However, many contributions to such a problem have been recently discussed in \cite{li2017extended, otto2019linearly, yeung2019learning, lusch2018deep}.
EDMD will be used to approximate a finite-dimensional Koopman operator based on a set of selected observables depending on the system.

Instead of having the system's states only, we consider additional observable functions as
${\Xi}({x}) = \begin{bmatrix}
    \xi_1({x}) & \xi_2({x}) & \dots & \xi_p({x})
\end{bmatrix}^{\top}.$ The observable functions ${\Xi} \in \mathbb{R}^{p} (p > n)$ are normally hard to infer and is still unclear which nonlinear observable functions are best to use for a given system and how doing so will affect the efficiency of approximation of the Koopman operator. 
The system in (\ref{eq:dmdc}) can simply become
\begin{align} 
    {\Xi(X^{+})} &= {A}{\Xi(X)} + {B}{\Gamma}\\
    &= \begin{bmatrix}
        {A} ~ {B}
    \end{bmatrix} \begin{bmatrix}
        {\Xi(X)}\\ {\Gamma}
    \end{bmatrix} = {\hat{\mathcal{K}_t}} {\bar{\Omega}},
    \label{eq:edmdc}
\end{align}
and a solution to this can be retrieved similar to what have been found in (\ref{eq:soln_ls}) with modified version to account for the lifted state as
\begin{align}
    \hat{\mathcal{K}_t} = \argmin_{{{\mathcal{K}_t}}} ||{\Xi({X}^{+})} - {\hat{\mathcal{K}_t}} \bar{\Omega}||_{\text{F}}.
    \label{eqn:normal_least_squares}
\end{align}


\begin{remark}
    If the used lifting functions are considered as identity, then the EDMD formulation simply reduces to the nominal DMD. \hfill $\Box$
\end{remark}
The linear lifted approximation of the nonlinear dynamics in (\ref{eq:dynamics}) can now be casted as
\begin{align*}
    z_{k}^{+} &= Az_{k} + Bu_{k}\\
    x_k & = Cz_{k}.
\end{align*}
% However, the solution given in (\ref{eq:soln_ls}) can be viewed as a least-squares solution to the problem given in (\ref{eq:dmdc}). This solution is known to have high sensitivity to noisy data. On the other hand, total-least-squares solution can mitigate the effect of noisy data as compared to the nominal least-squares. We lay the formulation of the total-least-squares solution to the same problem presented in the upcoming section for future usages.

% \subsection{Extended Dynamic Mode Decomposition with Total Least Squares}
% Here we use the total least squares algorithm to solve the EDMD problem. As discussed, the EDMD algorithm will be employed to approximate the Koopman operator. The algorithm will be used to solve the EDMD problem extended to account for controlled systems 
% motivated by the work cited  \cite{malioutov2014convex, williams2015data, golub1980analysis}. It can be used to get unbiased estimation of the Koopman operator. The total least squares method can be summarized as in \cite{hemati2017biasing} as follows:
% \begin{enumerate}
%     \item Calculate the Singular Value Decomposition (SVD) of the lifted data matrix as 
%     \begin{align}
%         \label{eqn:svd}\texttt{svd}\left(\begin{bmatrix}
%             \Xi({X})\\ \Xi({X^{+}})
%         \end{bmatrix}\right) = {U}{\Sigma}{V}^{*}.
%     \end{align}
%     \item Project the data matrices, calculating ${\bar{X}} = {X} {V} {V}^{*}$ and ${\bar{X}^{+}} = {X^{+}} {V} {V}^{*}$.
%     \item Do the normal DMD procedure on the projected data matrices.
% \end{enumerate}
% This solution makes it more robust towards the biased data. It is worth noting that the total least squares was developed on the nominal DMD formulation. We introduce the usage of total least squares to the EDMD formulation as encouraged by the authors of ref. \cite{hemati2017biasing}.

% The solution presented in (\ref{eq:soln_ls}) can be used after we project the data matrices and we call it a total-least-squares solution. This can also be viewed as a Frobenius norm minimization problem \cite{hemati2017biasing} as
% \begin{align}
%     \hat{\mathcal{K}_t} = \argmin_{{\hat{\mathcal{K}_t}}} ||{\Xi(\bar{X}^{+})} - {\hat{\mathcal{K}_t}} \bar{\Omega}||_{\text{F}}.
%     \label{eqn:normal_least_squares}
% \end{align}
% One also can constraint the problem more by adding a $L_1$ penalty norm term to account for sparsity of the approximated Koopman operator $\hat{\mathcal{K}}_t$ as
% \begin{align}
%     \hat{\mathcal{K}_t} = \argmin_{{\hat{\mathcal{K}_t}}} ||{\Xi(\bar{X}^{+})} - {\hat{\mathcal{K}_t}} \bar{\Omega}||_{\text{F}} + \lambda ||{\hat{\mathcal{K}_t}}||_{1},
%     \label{eqn:nuclear_norm}
% \end{align}
% where $\lambda \in \mathbb{R}^{+}$ is the weight of $L_1$ norm term. If we considered $\lambda = 0$, Eqn. (\ref{eqn:nuclear_norm}) reduces to the same least-squares solution as (\ref{eqn:normal_least_squares}). As $\lambda$ increases, $\hat{\mathcal{K}_t}$ becomes more sparse. The solution to (\ref{eqn:nuclear_norm}) is a trade off between the sparsity and complexity of the discovered operator from data (i.e. typical over-fitting/under-fitting problem). 
% \subsubsection{Problems with Dynamic Mode Decomposition Biasing}
% The sensitivity of the standard DMD algorithm's eigenvalue spectrum to noisy data is a significant problem. It has been demonstrated that when sensor noise is added to the data, there is a systematic bias in the eigenvalue spectrum that does not go away as more data is sampled \cite{bagheri2013effects, hemati2017biasing}. Such a problem is tackled in recent research. Dawson and his collaborators \cite{dawson2016characterizing}, processed the data in forward and backward time and data is then averaged, removing the systematic bias. Hemati et al.  \cite{hemati2017biasing} proposed to solve the DMD using total least squares algorithm to de-bias the DMD instead of the standard least squares .
The entire process of the proposed algorithm can be summarized in algorithm \ref{alg:koopman-identification}.
\begin{algorithm}[]
\caption{Koopman Identification using total-least-squares with $L_1$ regularization}
\label{alg:koopman-identification}
\begin{algorithmic}[1]
\REQUIRE $\lambda$, and dataset $\mathcal{D}$
\STATE  Lift data via (\ref{eqn:lift})
\STATE Get the approximated Koopman operator $\hat{\mathcal{K}}_t$ via (\ref{eqn:normal_least_squares})
\STATE  Extract the identified linear matrices $A$, $B$ from $\hat{\mathcal{K}}_t$
\RETURN $\hat{\mathcal{K}}_t$, $A$, and $B$
\end{algorithmic}
\end{algorithm}

\subsection{Quadcopter dynamics}
We assume the quadrotor is a rigid body with a 6 degrees of freedom with a mass $m$ and diagonal inertia tensor of ${J} = \text{diag(} J_{xx}, J_{yy}, J_{zz}\text{)}$. Our model is built upon  quaternion formulation for attitude parameterization and is similar to the standard models found in \cite{torrente2021data, carino2015quadrotor}. For better interpretation of the results we convert quaternions to Euler angles. The state space then is 13-dimensional or 12-dimensional respectively space, based on either quaternion, or Euler angles formulation (respectively). Suppose we deal with quaternion attitude formulation, so $x \in \mathbb{R}^{13}$ and is governed by the dynamics
\begin{align}
\label{eq:3d_quad_dynamics}
\dot{{x}} =
\deriv{}{t}\begin{bmatrix}
{{p}}_{WB} \\ 
\dot{{p}}_{WB} \\
{{q}}_{WB} \\
{\omega}_B
\end{bmatrix} = 
{f}({x}, {u}) =
\begin{bmatrix}
{p}_W \\ 
\frac{1}{m}\;{q}_{WB} \cdot {T}_B + {g}_W \\
\frac{1}{2} {q}_{WB} \otimes {\omega_B} \\
{J}^{-1}\left({\tau}_B - \omega_B \times {J}\omega_B\right)
\end{bmatrix},
\end{align}
where ${T}_B$ is the summation of quadrotor's thrust, ${g}_W= [0, 0, \SI{-9.81}{\meter\per\second^2}]^\top$ is Earth's gravity, ${\tau}_B$ is the torque, ${p}_{WB}$, position vector from world to body frame, and $q_{WB}$  quaternion from world to body frame. We also denote the quaternion-vector product by $\otimes$, where, for example, $p\otimes q = qp{q}^{*}$, and $q^{*}$ is the quaternion's conjugate. 
\begin{align}
{T}_B =  \mat{0 \\ 0 \\ \sum T_i} \quad
\text{and} \quad 
{\tau}_B = 
\mat{l (-T_0 - T_1 + T_2 + T_3) \\
l (-T_0 + T_1 + T_2 - T_3) \\
c_\tau (-T_0 + T_1 - T_2 + T_3)},
\end{align}
where $l$ is the distance from
the center of mass to the motor axis of action and $c_\tau$ is a constant for the rotor's drag torque.

We will consider the famous Runge-Kutta numerical integration scheme with order four to integrate the dynamics ${\dot{x}}$ in a discrete manner with a time step of $\Delta t$
\begin{equation}
\label{eq:discretized_nominal_dynamics}
{{x}_{k+1} = {x}_{k}} + \int_{k\Delta t}^{(k+1)\Delta t} {f}({x}, {u}, \Delta t) d \tau
\end{equation}
\subsection{Data Collection and Koopman Training}
A PD controller is designed to track the generated trajectories of the quadrotor. We simulated 5 helical trajectories with quadrotor's parameters in table \ref{tab:physical}, providing a diverse set of scenarios for analysis. 
\begin{table}[]
    \centering
    \caption{Physical parameters of the quadrotor}
    \label{tab:physical}
    \begin{tabular}{cc}
    \toprule
    \textbf{Parameter} & \textbf{Value} \\
      \midrule
      Mass $m$ (kg) & 0.18 \\
      Gravity $g \cdot \hat{{k}}$ (m/s\textsuperscript{2}) & 9.81 \\
      Inertia ${J}$ (kg$\cdot$m\textsuperscript{2}) & $\begin{bmatrix}
        0.00025 & 0 & 0 \\
        0 & 0.000232 & 0 \\
        0 & 0 & 0.0003738
      \end{bmatrix}$ \\
      Moment arm $l$ (m) & 0.086 \\
      \bottomrule
    \end{tabular}
\end{table}
A time step $\Delta t$ of $0.01$ seconds is set in the simulation to ensure detailed temporal resolution for 30 secendos for each trajectory. Random parameters are utilized to also introduce variability in the trajectories. The helix radius varies randomly between 1 and 5 meters, while the height experiences random fluctuations within the range of 1 to 6 units. We then transform the quaternions to Euler angles representing the attitude of the quadrotor.

We trained our EDMD model with total least squares optimizer dealing with the data using a set of observable from our background of the system and we augment it with another observable functions retrieved from literary sources (see ref. \cite{chen2022koopman}) defined as 
% \begin{equation}
%     \begin{aligned}
%         {\Xi}({x}) = \big[&1,~ p_{WB},~ \dot{p}_{WB}, ~ 
%         {x},~ \dot{{p}}_{WB}^{\top} {R}{R}^{\top}\dot{{p}}_{WB},~ \dots \\& T_2({x}),~ \sin({p}_{WB}),~ \cos({p}_{WB}),~ \dots \\ &{R}^{\top}\dot{{p}}_{WB},~ 
%          {{p}}_{WB} \times \dot{{p}}_{WB},~ {{p}}_{WB} \times  {\omega}_{B},~ \dots \\&{\omega}_{B} \times {\omega}_{B}, \text{vec}(R\hat{\omega}_{B})
%     \big] \in \mathbb{R}^{59},
%     \end{aligned}
% \end{equation}
\begin{equation} \label{eqn:lift}
    \begin{aligned}
        {\Xi}({x}) = \big[&1,~ x,~ p_{WB},~ \dot{p}_{WB},~ \sin(p_{WB}),~ \dots \\ & \cos(p_{WB}),~ \text{vec}(R \times \omega_{WB})
    \big],
    \end{aligned}
\end{equation}
where $\text{vec}(*): \mathbb{R}^{n\times n} \mapsto \mathbb{R}^{n^2 \times 1}$ is an operator that maps a matrix into a vector by stacking the columns of the matrix, and ${R}$ is the rotation matrix representing the quadrotor attitude. 

\subsection{Linear Quadratic Regulator Meets Koopman Linearization}
\begin{assumption} \label{ass:cont_obs}
    The identified pairs $(A, B)$ and $(A, C)$ are controllable and observable respectively. \hfill $\Box$
\end{assumption}
\begin{remark}
    Assumption \ref{ass:cont_obs} can be numerically verified for the identified system's matrices. \hfill $\Box$
\end{remark}
Now, consider a quadratic cost function:
\begin{align} \label{eqn:cost}
    \mathcal{J} = \minimize_{u_0,\dots,u_{N-1}} \sum_0^{N-1} x^{\top}(\tau)Qx(\tau) + u^{\top}(\tau)Ru(\tau) d\tau,
\end{align}
where $Q = Q^{\top} \succeq 0$ is a weight matrix for the cost of deviation of the state $x$ from the reference point, and $R = R^{\top} \succ 0$ weighs the cost of control action. If we considered a linearized version of (\ref{eq:dynamics}), it is possible to have a matrix $L$, and a control law in the form of $u = -Lx$ such that the cost $\mathcal{J}$ is minimum. However, this controller is linear, and in fact, it will be optimal only around the neighbourhood of the fixed point at which the linearization took place. \\
\indent Here, instead of having a local linear model for our system, we will instead use the global linear model derived from Koopman approximation. The cost function still holds but with minor modifications as follows
\begin{align*}
    \bar{Q} = \mat{Q_{n \times n} & 0_{p-n \times p-n}\\
    0_{p-n \times p-n} & 0_{p-n \times p-n}}_{p \times p}, \quad \bar{R} = R
\end{align*}
So, in cost function given in (\ref{eqn:cost}), we will replace $x$ by $z$, and $Q$ by $\bar{Q}$.
\begin{remark}
    In this formulation, the matrix $R$ stay as it is as we do not lift the control input. \hfill $\Box$
\end{remark}
In that sense, we can design an optimal LQR controller for our koopman linearization of our system. \\
\indent We choose $Q = \mathbb{I}_{12 \times 12} \times 10^{3}$, and $R = \mathbb{I}_{4 \times 4}$. Then we compare out strategy with a nominal PID controller. Results of both techniques will be discussed in details in the upcoming sections.
